A Local Discontinuous Galerkin Level Set Reinitialization with Subcell Stabilization on Unstructured Meshes

In this paper we consider a level set reinitialization technique based on a high-order, local discontinuous Galerkin method on unstructured triangular meshes. A finite volume based subcell stabilization is used to improve the nonlinear stability of the method. Instead of the standard hyperbolic level set reinitialization, the flow of time Eikonal equation is discretized to construct an approximate signed distance function. Using the Eikonal equation removes the regularization parameter in the standard approach which allows more predictable behavior and faster convergence speeds around the interface. This makes our approach very efficient especially for banded level set formulations. A set of numerical experiments including both smooth and non-smooth interfaces indicate that the method experimentally achieves design order accuracy.

==> figures/tikz_fv_storage.tex <==
% \documentclass{article}
% % main document, called main.tex
% \usepackage{tikz}
% \usetikzlibrary{external}
% \tikzexternalize % activate!
% \begin{document}


% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: 
\path (0,400); %set diagram left start at 0, and has height of 400
%Flowchart: Connector [id:dp36334759955028506] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (194,183) .. controls (194,180.24) and (196.24,178) .. (199,178) .. controls (201.76,178) and (204,180.24) .. (204,183) .. controls (204,185.76) and (201.76,188) .. (199,188) .. controls (196.24,188) and (194,185.76) .. (194,183) -- cycle ;
%Flowchart: Connector [id:dp8653833555960755] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (269,227) .. controls (269,224.24) and (271.24,222) .. (274,222) .. controls (276.76,222) and (279,224.24) .. (279,227) .. controls (279,229.76) and (276.76,232) .. (274,232) .. controls (271.24,232) and (269,229.76) .. (269,227) -- cycle ;
%Flowchart: Connector [id:dp08526177209282815] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (119,227) .. controls (119,224.24) and (121.24,222) .. (124,222) .. controls (126.76,222) and (129,224.24) .. (129,227) .. controls (129,229.76) and (126.76,232) .. (124,232) .. controls (121.24,232) and (119,229.76) .. (119,227) -- cycle ;
%Flowchart: Connector [id:dp6874435430624763] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (194,97) .. controls (194,94.24) and (196.24,92) .. (199,92) .. controls (201.76,92) and (204,94.24) .. (204,97) .. controls (204,99.76) and (201.76,102) .. (199,102) .. controls (196.24,102) and (194,99.76) .. (194,97) -- cycle ;
%Straight Lines [id:da9940553029697292] 
\draw    (348,270) -- (48,270) ;
%Straight Lines [id:da5950697408123997] 
\draw    (199.62,10.19) -- (48,270) ;
%Straight Lines [id:da46866012450159666] 
\draw    (199.62,10.19) -- (348,270) ;
%Straight Lines [id:da9978103716213578] 
\draw    (123.81,140.1) -- (198,270) ;
%Straight Lines [id:da5433918254300527] 
\draw    (123.81,140.1) -- (273.81,140.1) ;
%Straight Lines [id:da8973321401800765] 
\draw    (273.81,140.1) -- (198,270) ;
%Shape: Rectangle [id:dp44333340219292294] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (343,265.5) -- (353,265.5) -- (353,274.5) -- (343,274.5) -- cycle ;
%Shape: Rectangle [id:dp776353397622314] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (194.62,5.69) -- (204.62,5.69) -- (204.62,14.69) -- (194.62,14.69) -- cycle ;
%Shape: Rectangle [id:dp05701645899113017] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (268.81,135.6) -- (278.81,135.6) -- (278.81,144.6) -- (268.81,144.6) -- cycle ;
%Shape: Rectangle [id:dp009972070653662346] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (118.81,135.6) -- (128.81,135.6) -- (128.81,144.6) -- (118.81,144.6) -- cycle ;
%Shape: Rectangle [id:dp5507449511947009] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (44,265.5) -- (54,265.5) -- (54,274.5) -- (44,274.5) -- cycle ;
%Shape: Rectangle [id:dp5807100659462046] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (193,265.5) -- (203,265.5) -- (203,274.5) -- (193,274.5) -- cycle ;


% Text Node
\draw (205,145) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\overline{\phi }_{i}^{0}$};
% Text Node
\draw (128,192) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\overline{\phi }_{i}^{1}$};
% Text Node
\draw (275,189) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\overline{\phi }_{i}^{2}$};
% Text Node
\draw (205,61) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\overline{\phi }_{i}^{3}$};
% Text Node
\draw (141,140) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle S_{i}^{0}$};
% Text Node
\draw (67,233) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle S_{i}^{1}$};
% Text Node
\draw (218,232) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle S_{i}^{2}$};
% Text Node
\draw (185,30) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle S_{i}^{3}$};


\end{tikzpicture}
% \end{document}
